Improving Activation Steering in Language Models with Mean-Centring

Recent work in activation steering has demonstrated the potential to better control the outputs of Large Language Models (LLMs), but it involves finding steering vectors. This is difficult because engineers do not typically know how features are represented in these models. We seek to address this issue by applying the idea of mean-centring to steering vectors. We find that taking the average of activations associated with a target dataset, and then subtracting the mean of all training activations, results in effective steering vectors. We test this method on a variety of models on natural language tasks by steering away from generating toxic text, and steering the completion of a story towards a target genre. We also apply mean-centring to extract function vectors, more effectively triggering the execution of a range of natural language tasks by a significant margin (compared to previous baselines). This suggests that mean-centring can be used to easily improve the effectiveness of activation steering in a wide range of contexts.

==> content-4-page.tex <==
\begin{abstract}
Recent work in activation steering has demonstrated the potential to better control the outputs of Large Language Models (LLMs), but it involves finding steering vectors. 
This is difficult because engineers do not typically know how features are represented in these models. 
We seek to address this issue by applying the idea of \emph{mean-centring} to steering vectors. We find that taking the average of activations associated with a target dataset, and then subtracting the mean of all training activations, results in effective steering vectors. 
We test this method on a variety of models on natural language tasks by steering away from generating toxic text, and steering the completion of a story towards a target genre.
We also apply mean-centring to extract function vectors, more effectively triggering the execution of a range of natural language tasks.
\end{abstract}

\section{Introduction}

% Motivation + comparison to image models.

Large Language Models (LLMs) have become increasingly capable over the past few years across a diverse range of tasks \cite{peters2018deep, radford2019language, openai2023gpt4}.
% However, they are in many senses black-box models, which prevents us from addressing issues such as social biases and potential misuse.
However, in part due to a lack of understanding of how these capabilities are implemented, we are unable to address issues such as social biases \cite{abid2021persistent}.
Some approaches to mitigating these issues modify the weights of the LLM \cite{ilharco2023editing, meng2022locating}, but these techniques either require fine-tuning or have only been applied to editing factual associations encoded in the model.
% Mean-Centred Activation Steering is best understood as generalising the Activation Addition method proposed by \cite{turner2023activation}, as outlined in Section \ref{sec:methods}. 

A recent approach to controlling LLMs is \textit{activation steering} \cite{turner2023activation, li2023inferencetime, subramani2022extracting}, or similarly \textit{representation engineering} \cite{zou2023representation}. 
Activation steering aims to extract features from language models to better control their outputs. It typically does this by making inference-time modifications to some activations of the model. 

% Recent work known as \textit{representation engineering} unified these approaches \cite{zou2023representation}.
% One pertinent example from this area is the identification of directions in residual stream space that correspond to truth \cite{burns2022discovering}, allowing \citet{li2023inferencetime} to implement activation steering that improves language model truthfulness.
% This utilises entire datasets similarly to our methods, but focuses on attention heads and not MLP layers.
% \citet{subramani2022extracting} compute steering vectors that successfully increase the probability of desired target sentences, although it's not clear if this could generalise to creating steering vectors for broader features.

% Our investigations into understanding and using latent space representations of language models follow from similar findings regarding other architectures \cite{word2vec, radford2017learning}, extending this to transformer networks. 

% \citet{} discover a single neuron in an LSTM which controls the sentiment of a movie review. Our work provides an analogous method for transformer networks, and can also be used to find arbitrary feature representations.
% \citet{ilharco2023editing} present an alternative method of generating steering vectors to change the behaviour of language models, by finding directions in weight-space. This required fine-tuning, which is more compute intensive than Mean-Centred Activation Steering which only requires running inference on the model. \citet{meng2023locating} also intervenes on model weights to change the behaviour of language models, although they focus on editing specific factual associations instead of features.


% Although there have been some promising initial results in activation steering, there are difficulties that still need to be overcome in order to apply it more widely. 
% One such difficulty is the current lack of understanding of the activations of these models, which makes it difficult to know in which direction to steer activations.

In this work, we apply activation steering to make a language model incorporate some behaviour exhibited by an arbitrary dataset $D$. 
This would introduce a simple pipeline for modifying language model behaviour, but current activation steering methods do not allow for this in full generality. 
They either require the identification of an opposite behaviour (Counterbalanced Subtractions in \citet{turner2023activation}), succinctly describing the pertinent behaviour of the dataset (LAT Scans in \citet{zou2023representation}), or are computationally expensive (training a sparse autoencoder on language model activations \cite{cunningham2023sparse, bricken2023monosemanticity}).



 Our paper aims to address these issues by applying a simple processing technique to steering vectors, in the spirit of similar work in word representations \cite{mu2018all}. 
 Our technique, which we call \emph{mean-centring}, successfully incorporates properties of datasets into the outputs of LLMs, whilst maintaining coherence.
 This provides a simple method for changing model behaviour using only a dataset, making it easier to apply activation steering in a wider range of contexts. In summary:

\begin{itemize}
    % \item We extend the anisotropy result to other models, i.e. language model activations typically have a non-zero mean.
    %, and hypothesise why this could prevent naive methods of forming steering vectors using datasets.
    \item In Section \ref{sec:method} we introduce mean-centring as a method for creating better steering vectors. 
    % This method is motivated by anisotropy results that we extend.
    %This method is an improvement because 1) it creates better results; and 2) can be applied to a wider range of tasks. 
    \item In Section \ref{sec:toxicity-results} we demonstrate the efficacy of mean-centring by controlling a language model to generate non-toxic continuations of toxic comments.
    \item In Section \ref{sec:story-results} we show that mean-centring increases the range of tasks for which steering can be applied as compared to methods that require a counterbalancing concept. We demonstrate the efficacy of mean-centring by influencing the genres of stories as they are generated.
    \item In Section \ref{sec:function-vectors} we demonstrate the efficacy of mean-centring by extracting more effective function vectors, compared to non mean-centred approaches.
\end{itemize}

\begin{figure}[h]
\centering
\includegraphics[width=0.7\linewidth]{figures/mean-centring-aaai.png}
\caption{An example of mean-centring illustrated on a set of highly anisotropic activations (i.e. offset from the origin). 
When steering, we want to use the vector $\mathbf{f}$ which generates some target behaviour. This can be extracted by averaging activations from a dataset exhibiting this behaviour, $\mu_{\text{target}}$, if we account for the mean across all training examples $\mathbf{b}$. 
% If all activations are distributed about bias vector $b$, and there exists some activations associated with loving text, then just taking the mean of the loving activations will produce $b + f$ vector. The vector $f$ can be isolated by subtracting the bias vector $b$.
}
\label{fig:zero-v-mean-act}
\end{figure}


 
 % We empirically demonstrate the efficacy of our method by controlling language models to generate non-toxic continuations of toxic comments and to influence the genre of a story being generated.


% \begin{figure}[!h]
%     \includegraphics[width=\textwidth]{figures/smile.png} 
%     \caption{After finding how smiles were represented in GAN models, it was possible to introduce the smile feature to output images. Image from \cite{white2016sampling}.}
% \end{figure}


\section{Related Work}

% In Section \ref{sec:lin-rep-hyp} we introduce some intuitive explanation for why activation steering works; in Section \ref{sec:act-steering} we give a brief overview of the nascent field of activation steering and in Section \ref{sec:anisotropy} we discuss anisotropy in residual stream activations.

\subsection{Linear Representation Hypothesis}\label{sec:lin-rep-hyp}
The \emph{linear representation hypothesis} \cite{elhage2022superposition} proposes that many human-interpretable high-level concepts are represented linearly as directions in the residual stream of language models. 
% Since attention heads and MLP layers add to the residual stream, this hypothesis also proposes that human-interpretable concepts are represented as directions in their outputs.   % cite https://arxiv.org/abs/2311.03658
There is significant evidence for the linear structure of neural network representations, including linear operations on Word2Vec embeddings capturing semantic meaning \cite{word2vec}. 
There is  strong evidence in the context of language models specifically, due to the success of linear probes and edits locating information within models \cite{meng2022locating, nanda2023emergent, gurnee2023language}.
Recent advances in learning the representations of concepts in language models using sparse auto-encoders provides substantial further evidence for this hypothesis \cite{cunningham2023sparse, bricken2023monosemanticity}.
% For the purpose of this paper we will call directions in the representation space \emph{features}.

This suggests that if we find the right vector to represent a concept, then we can steer any residual stream activation into the direction of that concept by simply adding that vector to the activation \cite{zou2023representation}.
% In contrast, if the hypothesis were not true, concepts could be represented as regions in the residual stream space, and thereby the steering vector would need to change depending on the current activation. 
% This issue has been identified in the context of feed-forward neural networks \cite{polytope-lens}, but has not been identified in language models.

% Monosemanticity/Hoagy paper found  that interpretable features are represented in hidden layer activations (these can be extracted using sparse auto-encoders). 

% Supporting this finding, in Appendix \ref{app:more-empirical} we show via t-SNE plots that genres are represented in the residual stream activations. 

% + cosine similarity graphs imply anisotropic representations in the res stream

% + directions don't reduce representational capacity as the probability of conflicts 

% The above suggests that there exist regions of space that correspond to certain features, but it doesn't provide evidence about how features will be represented in language models. To progress here, we use the \textit{Linear Representation Hypothesis} \cite{elhage2022superposition}: in some layer $l$, language models represent some target feature as a direction in residual stream space, $f^{l}_{target}$. 


\subsection{Activation Steering}\label{sec:act-steering}
There have been recent efforts to control the outputs of language models through \textit{activation steering}, i.e. adding vectors into the activations of a model at inference time. 
The general aim of activation steering is to introduce some property into the output of a model by identifying some steering vector $\mathbf{f}$ and adding it to some layer(s) of the forward pass of a model, at some token position(s). 
This has been applied to incorporating features such as how ``loving" a text is \cite{turner2023activation}, functions such as reciting the capital of a country \cite{todd2023function}, and improving the truthfulness of text \cite{li2023inferencetime}.  


% Our work primarily builds on \citet{turner2023activation}, who provided a general method for performing activation steering by using arbitrary text inputs to create steering vectors. We discuss how \citet{turner2023activation} create steering vectors when we contrast it to our approach in Section \ref{sec:methods}. 

% It requires a steering vector $\mathbf{f}_{target}^l$ to be identified, along with two main hyperparameters: a layer $l$ to add the steering vector to, and a strength coefficient $\steeringcoef$ that controls the magnitude of the effect. During activation steering the model then runs a typical forward pass, except for adding to the activations at a single layer via  \(x'_{l} = x_{l} + \steeringcoef \mathbf{f}_{target}^{*l}\). Here $\mathbf{f}_{target}^{*l}$ is a padded version of $\mathbf{f}_{target}^{l}$ to allow us to apply it to the entire tensor instead of a single vector.

% We extend this method by finding new methods for creating steering vectors. 

% \subsection{Extracting Representations from Datasets}
% Various methods exist for extracting representations from 

In this paper we will always add a steering vector $\textbf{f}$ to the final token position, and at a single layer.

\subsection{Anisotropy}\label{sec:anisotropy}
An alternative way of understanding the activations of language models comes from analysing their geometric structure. 
Multiple works have demonstrated the \textit{anisotropy} of the activations of language models \cite{ethayarajh2019contextual,cai2021isotropy}.
Anisotropic activations are not distributed uniformly around the zero point in activation space, but instead are offset in a consistent direction. 
A similar phenomena was also identified in classical word representations in NLP such as word2vec \cite{word2vec} and GLoVE \cite{pennington2014glove}. \citet{mu2018all} improve downstream performance on these word representations by subtracting the mean, and then projecting on the dominant remaining directions. This directly inspires our own method of mean-centring.

% Although the phenomena isn't fully understood, \cite{gao2019representation} has presented one theoretical explanation for anisotropy based on the combination of LayerNorm and weight-tying.


% Although there are further complexities to the structure of activation space than just anisotropy \cite{cai2021isotropy}, this insight can help to better describe the activations of these models.

\section{Mean-Centred Activation Steering}
\label{sec:method}



\begin{algorithm}[t]
\caption{Mean-Centred Activation Steering ($\mu$ActAdd)}\label{alg:mean-centring}
\hspace*{\algorithmicindent} \textbf{Input}:  \\
\hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $M$ = language model \\
\hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $p$ = user prompt \\
% \hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $n$ = maximum output length \\
\hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $\mathcal{D}_{\text{training}}$ = training dataset sample \\
\hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $\mathcal{D}_{\text{target}}$ = target dataset \\
% \hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $c$ = injection coefficient \\
% \hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $l$ = target layer \\
% \hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $f$ = distillation vector extender
\hspace*{\algorithmicindent} \hspace*{\algorithmicindent}SteeringMethod = Method used to steer language model

\hspace*{\algorithmicindent} \textbf{Output}: \\
\hspace*{\algorithmicindent} \hspace*{\algorithmicindent} $S$ = steered output text

% \hspace*{\algorithmicindent} \textit{Calculate the mean of the feature activations}:
\begin{algorithmic}[1]
% \FOR{$1 \leq i \leq N$} 
%     \STATE $\mathbf{h}_{i}$ $\leftarrow$ $M$.forward($x_{i}$).activations[$l$]
%     \STATE $\mathbf{\Bar{x}} \leftarrow \mathbf{\Bar{x}} * \frac{i-1}{i} +  \mathbf{h}_{i} * \frac{1}{i}$
% % Check this is the moving average formula lmao
% \ENDFOR

% \textit{\\}
% \textit{Calculate the mean of the baseline activations}

% \FOR{$1 \leq i \leq N'$}
%     \STATE $\mathbf{h'}_{i}$ $\leftarrow$ $M$.forward($x'_{i}$).activations[$l$]
%     \STATE $\mathbf{\Bar{x}'} \leftarrow \mathbf{\Bar{x}'} * \frac{i-1}{i} +  \mathbf{h'}_{i} * \frac{1}{i}$
% % Check this is the moving average formula lmao
% \ENDFOR

% \textit{\\}
% \textit{Calculate the steering vector}
\STATE $M.forward(\mathcal{D_\text{target}})$
\STATE $\mu_{target} = \text{Mean}(M.activations)$
\STATE $M.forward(\mathcal{D_\text{training}})$
\STATE $\mu_{training} = \text{Mean}(M.activations)$
\STATE $\mathbf{v} \leftarrow \mu_{target} - \mu_{training}$

% \textit{Autoregressively produce output using the steering vector}

\STATE $ S \leftarrow$ SteeringMethod(M,p,$\mathbf{v}$)

% \FOR{$i \leq n$}
%     \STATE $\mathbf{v'} = f(\mathbf{v}, S)$
%     \STATE $\mathbf{x}_{l}$ $\leftarrow$ $M$.forward($S$).activations[$l$]
%     \STATE $t \leftarrow $ $M$.continueForward($c\mathbf{v'} + \mathbf{x}_{l}$).text
%     \STATE $S \leftarrow S$.append($t$)
% \ENDFOR

% Make it clearer where activations are add (front / back / everywhere)
% Explain the three sections more clearly.
\end{algorithmic}
\label{alg:act-add}
\end{algorithm}


% A variety of neural networks are able to recognise and represent features of text in their latent spaces \cite{word2vec, radford2017learning}. 
% This inspired new methods of interpreting language models known as representation engineering \cite{zou2023representation}, which identifies a broad framework for reading and controlling the feature representations used by language models. 
% Although this was focused on reading and controlling feature representations related to concepts such as honesty and morality, there has been further work demonstrating that language models represent some functions as features \cite{todd2023function}.

% Intuitively, a feature $\mathcal{F}$ of some input text is some property of the text which can be present in varying degrees. 
% A formal definition, based on \cite{ilyas2019adversarial}, is that a feature $\mathcal{F}$ is a function mapping from the input space $\mathcal{X}$ to the positive real numbers $\mathbb{R^{+}}$. 
% For some text input $s$, we can therefore interpret $\mathcal{F}(s)$ as the degree to which the feature $\mathcal{F}$ is present in the input $s$, with $\mathcal{F}(s) = 0$ meaning the feature $\mathcal{F}$ is entirely absent from the input $s$.

% For example of a feature of some text $s$ might be a function that maps to $1$ if an animal is described in the text, and $0$ otherwise. This description is broad enough that any attribute of text can be described formally as a feature this way.



% A natural question is to then ask how model's represent features in their activations. 
The method that we propose aims to get an LLM to exhibit behaviours that are not well-defined, but that can be captured by a dataset of examples that demonstrate the behaviour.
Therefore, in our method we use a \emph{target dataset} made of examples of a target behaviour to extract a \emph{distillation vector} that can be used to get an LLM to generate the target behaviour.

Let $\mathbf{x}_{1}, \ldots, \mathbf{x}_{n}$ be the residual stream activations at some layer $l$ across all token positions of an LLM when performing inference on a target dataset $\mathcal{D}_{\text{target}}$ of exemplary behaviour. 
From the set of activations $\mathbf{x}_{1}, \ldots, \mathbf{x}_{n}$ we want to extract a distillation vector $\mathbf{f}$.
Previous work \cite{cai2021isotropy} has demonstrated that the activations of GPT-2 Small and BERT activations typically have a non-zero mean (Section \ref{sec:anisotropy}), across all layers. 
In Appendix \ref{app:bias} we replicate these findings for state-of-the-art open-source models including GPT-2 XL \cite{radford2019language}, GPT-J \cite{gpt-j},  and Llama-2 \cite{touvron2023llama}.
This means that we might decompose the activations $\mathbf{x}_{i}$ as
\begin{equation}
 \mathbf{x}_{i} = \alpha_{i}\mathbf{f} + \mathbf{b} + \mathbf{v}_{i},
\end{equation}
where $\mathbf{f}$ is the representation of the behaviour displayed in the dataset $\mathcal{D}_{\text{target}}$, $\mathbf{b}$ is the bias vector applied to all activations in the language model, and $\mathbf{v}_{i}$ is a noise vector encoding information about behaviour not shared by the other datapoints in $\mathcal{D}_{\text{target}}$.
The mean of these activations can now be described 
\begin{equation}
\mu_{target} :=  \frac{1}{n}\sum_{i=1}^{n}\alpha_{i}\mathbf{f} + \frac{1}{n}\sum_{i=1}^{n}\mathbf{v}_{i} + \mathbf{b} . 
\end{equation}
If we assume that the noise vectors, $\mathbf{v}_{i}$, are distributed independently about the $\mathbf{0} \in \mathbb{R}^{d_{\text{model}}}$ vector, 
then by the law of large numbers the mean of all activations $\mathbf{x}_i$ becomes
\begin{equation}\label{eq:bias}
    \mu_{target} \rightarrow \alpha \mathbf{f} + \mathbf{b} \hspace{0.5cm}\text{ as }\hspace{0.5cm} n \rightarrow \infty.  
\end{equation}

Steering with $\mu_{target}$ directly might be sub-optimal, since the bias vector $\mathbf{b}$ in Equation \ref{eq:bias} has significant magnitude and does not encode any information specific to the dataset $\mathcal{D}_{\text{target}}$. We demonstrate its ineffectiveness empirically in Section \ref{sec:results}.

% Introducing more of the bias vector $\mathbf{b}$ than is normally present in the activations, which may degrade performance. 

% We present a simple solution to this problem, based on the idea of mean-centring used frequently in interpretability work (cite causal scrubbing etc.).

% Due to the inspiration from similar approaches in other contexts such as causal scrubbing \cite{causal-scrubbing}.

Instead, we remove the bias vector $\mathbf{b}$ from $\mu_{target}$. Assuming that averaging activations $\mathbf{x}'_{1}, \ldots, \mathbf{x}'_{n'}$ of samples of the training distribution, $\mathcal{D}_{\text{training}}$, approximates $\mathbf{b}$:
\begin{equation}
    \mu_{training} := \frac{1}{n'}\sum_{i=1}^{n'}\mathbf{x}'_{i} \approx \mathbf{b},
\end{equation}
allows us to extract the vector via $\mathbf{f} \approx \mu_{target} - \mu_{training}$. 

% Hence, a more accurate description of the activations might be \( \mathbf{x}_{l,i} = \mathbf{f}^{l}_{target} + \mathbf{\mu^{l}_{all}} + \mathbf{e}'_{l,i}\).
% Assuming that the $\mathbf{e}'_{l,i}$ vectors are independently distributed about the $\mathbf{0} \in \mathbb{R}^n$ vector, this gives the mean as:
% \begin{align}
% \mu_{target}^{l} = \mathbf{f}^{l}_{target} + \mu^{l}_{all} + \frac{1}{k}\sum_{i=1}^{k} \mathbf{e}'_{l,i}
% \rightarrow \mathbf{f}^{l}_{target} + \mu^{l}_{all}
% \end{align}
% as \( k \rightarrow \infty \) (i.e., as we grow our dataset of target feature examples). To approximate the vector $\mathbf{f}^{l}_{target}$, the activations can be \textit{mean-centred} by approximating the bias $\mu^{l}_{all}$ via sampling the training dataset and then subtracting this from $\mu^{l}_{target}$.

% If the dataset contains other unwanted correlates that we do not want to extract, these can be removed by subtracting a vector corresponding to the bias direction and the unwanted correlates too. 
% Make the above more explicit, but also keep it brief.

We call this method of extracting distillation vectors \textit{mean-centring}, which we illustrate in Figure \ref{fig:zero-v-mean-act}.
We present the algorithm used to implement mean-centred activation steering in Algorithm \ref{alg:mean-centring}.

% \section{Experimental Set-Up}

% \subsection{Models}
% We will limit our analysis to decoder-only, GPT-2 \cite{radford2019language} style language models, in particular the GPT-2 Small and XL models available through Transformer Lens \cite{nandatransformerlens2022}. These models first embed the input, $\mathbf{x}_{0}$, which forms the start of the \textit{residual stream}. This is a sequence of tensors $\mathbf{x}_{0},...,\mathbf{x}_{n}$, which successive transformer blocks read from and write to, via $\mathbf{x}_{l+1} = t_{l}(\mathbf{x}_{l}) + \mathbf{x}_{l}$.

% \subsection{Datasets}

\section{Experimental Evaluations}
\label{sec:results}

In this section we evaluate mean-centring in three different contexts. We firstly evaluate its effectiveness at removing toxicity from language models (Section \ref{sec:toxicity-results}), demonstrating that it is comparable to an existing steering method, namely counterbalanced subtractions from \citet{turner2023activation}. We then apply mean-centring to two domains where techniques like counterbalanced subtractions or LAT Scans are not applicable: steering the genre of stories (Section \ref{sec:story-results}) and extracting better function vectors (Section \ref{sec:function-vectors}). 
In Appendix \ref{app:datasets} we discuss the datasets that we use in this section.
% To do if there's time: include a small appendix for the models that we us
% GPT-2 Small, GPT-2 XL, GPT-J 6B 
% In a future version, maybe LLama-2 7B

\subsection{Removing Toxicity Experiments}
\label{sec:toxicity-results}
In this section we demonstrate the efficacy of mean-centring in reducing the toxicity of language models. We prompt GPT-2 Small to generate continuations of toxic comments, 
where prompts are created using a derivative of the Jigsaw Toxic Comments dataset \cite{jigsaw-toxic-comment-classification-challenge, borkan2019nuanced} that only included  toxic comments (Appendix \ref{app:dataset-toxic}\footnote{Warning: examples of offensive and hateful comments appear in the Appendix, but none appear in the main paper contents}). We took the first half of each comment and used GPT-2 Small to generate continuations, using each of the following methods of steering:
\begin{itemize}
    \item Mean-centring (Non-Toxic): Using mean-centring with a dataset of `non-toxic' text, a subset of the Jigsaw dataset filtered to only include non-toxic comments.
    \item Mean-centring (Loving): Using mean-centring with the Loving dataset containing `loving' text generated by GPT-3.5 (Appendix \ref{app:dataset-loving} for details of this dataset). 
    \item No-centring (Loving): Using the average of the activations associated with the Loving dataset (Appendix \ref{app:dataset-loving}), but without mean-centring.
    \item ActAdd: Using the ActAdd method from \citet{turner2023activation} with the prompt `Love' counterbalanced by `Hate'.
    \item Unsteered: Standard inference.
\end{itemize}


To evaluate the generated text, we use two pretrained models trained to classify positive sentiment and toxicity separately. 
First, we use a DistilBERT \cite{Sanh2019DistilBERTAD} model with a sentiment head trained on the Stanford Sentiment Treebank (SST-2) dataset \cite{socher-etal-2013-recursive} to compute positive sentiment values. % TODO: The appendix provides evidence that the model retains capabilities, in the sense that steering doesn't significantly reduce the relevance of the model's responses.
Second, we use a RoBERTa model \cite{liu2019roberta} trained on the Jigsaw dataset to classify toxicity \cite{dale2021skoltechnlp}.
% nother pretrained model, this time trained to classify the toxicity of a given sample of text. This was a RoBERTa model\cite{liu2019roberta} trained to predict whether a comment from the Jigsaw dataset was toxic or not \cite{dale2021skoltechnlp}. 
We take the log-probability of being classified as `toxic' to evaluate the toxicity of a text. 
We perform a hyperparameter sweep that minimises toxicity to fairly compare the methods (see Appendix \ref{app:toxicity-hyperparams} for details).

Once the best hyperparameters have been selected, Figure \ref{fig:toxicity} displays the results of the final steering methods.
Figure \ref{fig:sentiment} shows the average sentiment and Figure \ref{fig:toxicity_boxplot} shows the negative toxicity log-probability of generated text, a higher value respectively represents more positive sentiment and lower toxicity.
We find that for both average sentiment and negative toxicity log-probability, the mean-centring (Loving) method is superior to all other methods we investigate, and in particular to the no-centring (Loving) method.
We also find that the mean-centring (Non-Toxic) method is able to reduce the toxicity of the model without substantially increasing the sentiment of responses.
This demonstrates that one can control mean-centring steering methods effectively by choosing appropriate datasets.


% Figure \ref{fig:sentiment} shows that the sentiment of the generated text improves significantly with the Mean-Centred (Loving) method, more than when using the ActAdd method or the No-Centring method. Both display more positive sentiment than the unsteered completions. 
% Figure \ref{fig:toxicity_boxplot} shows that the Mean-Centred (Loving), Mean-Centred (Non-Toxic), and ActAdd methods produce substantially less toxic outputs than the Unsteered and No-Centring (Loving) methods, providing significant evidence of the performance of these methods.
Appendix \ref{app:steering-examples} includes examples of steered comment completions using the different methods.

% \begin{figure}[t]
%   \begin{minipage}[b]{0.48\linewidth}
%     % \includegraphics[width=\linewidth]{figures/sentiments-2023-09-29 15_51_46.726272.pdf}
%     \includegraphics[width=.8\linewidth]{figures/steered-vs-unsteered-toxic-comment-sentiments.pdf}
%     \caption{Change in average sentiment with each word generated of the unsteered and steered toxic comment completions.}
%     \label{fig:sentiment}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.48\linewidth}
%   \centering
%   % \footnotesize
%   \tiny
%     \begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
%       \hline
%       Unsteered & Steered Response \\
%       \hline
%       \textbf{Jehovah's Witnesses are a bunch of cultish FREAKS and they need to go ahead and drink the `kool-aid'} for them. They don't even know what they're doing. You can find the video here: [link] And you can also check out this video from an interview with one of Jehovah's Witnesses who is now in jail: [link]  & \textbf{ Jehovah's Witnesses are a bunch of cultish FREAKS and they need to go ahead and drink the `kool-aid'} (whatever) that makes them happy. The reason for this is because of their love for the Lord, who loves them, and loves their soul. 
%       They also believe in God and love his perfect body, which is perfect in all but His glory. I have seen your face. I have seen your life filled with joy; I have loved you with my heart, my love has been yours forever
%       \\
%       \hline
%     \end{tabular}
%     \centering
%     % \vspace{.5cm}
%     \vspace{.5cm}
%     \caption{An example of applying the Mean-Centred Steering to a toxic comment using the ``loving text'' distillation vector.}
%     % \vspace{.375cm}
%   \end{minipage}
% \end{figure}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.467\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/toxicity/steered-vs-unsteered-toxic-comment-sentiments-shorter-draft-2023-12-01-21-46-09.pdf}
        \caption{Changes in mean positive sentiment of generated text with each word generated for the different methods (with 95\% CI bands).} \label{fig:sentiment}
    \end{subfigure}
    % \hfill
    % \hspace{.25cm}
    % \vspace{0.5cm}
    \begin{subfigure}{0.467\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/toxicity/toxicity-barplot-2023-12-01-21-59-01.pdf}
        \caption{Negative toxicity log-probabilities for the different steering methods (higher means less toxic), showing toxicity reductions for mean-centred steering and ActAdd \cite{turner2023activation}.} \label{fig:toxicity_boxplot}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{Results from Toxicity Removal Experiments} \label{fig:toxicity}
    % \vspace{-0.2cm}
\end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/genre-steering/combined_plots-2023-12-01-20-50-06.pdf}
    % \vspace{-0.6cm}
    \caption{Genre-word frequencies in generated text continuing stories of a given genre. Text generated without steering (Unsteered) is compared to text generated using mean-centring with a target genre's dataset (Mean-centred). Mean-centring consistently reduces the frequency of words in the genre we are steering away from, and increases the frequency of words in the genre we are steering towards.}
    \label{fig:story-continuations}
    \vspace{-0.3cm}
\end{figure}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{.45\textwidth}
        \centering
        \includegraphics[height=3.5cm]{figures/function_vectors/gptj-steered-accuracy-more-layers2023-12-01-21-06-32.pdf}
        \caption{Average accuracy across 6 different tasks for each layer.}
        \label{fig:FV-layers}
    \end{subfigure}%
    \begin{subfigure}{.45\textwidth}
        \centering
        \includegraphics[height=3.5cm]{figures/function_vectors/gptj-steered-accuracy-layer152023-12-01-21-07-38.pdf}
        \caption{Steering in Layer 15 for each task (5 random seeds).}
        \label{fig:FV-layer15}
    \end{subfigure}%
    % \vspace{-0.1cm}
    \caption{Average accuracy (with 95\% CI error bars) plots for steering GPT-J with the uncentred and mean-centred method.}
    % \vspace{-0.4cm}
\end{figure*}



% \begin{figure}[t]
%   \begin{minipage}[b]{0.48\linewidth}
%     % \includegraphics[width=\linewidth]{figures/sentiments-2023-09-29 15_51_46.726272.pdf}
%     \includegraphics[width=.8\linewidth]{figures/steered-vs-unsteered-toxic-comment-sentiments.pdf}
%     \caption{Change in average sentiment with each word generated of the unsteered and steered toxic comment completions.}
%     \label{fig:sentiment}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.48\linewidth}
%   \centering
%   % \footnotesize
%   \tiny
%     \begin{tabular}{|p{0.45\linewidth}|p{0.45\linewidth}|}
%       \hline
%       Unsteered & Steered Response \\
%       \hline
%       \textbf{Jehovah's Witnesses are a bunch of cultish FREAKS and they need to go ahead and drink the `kool-aid'} for them. They don't even know what they're doing. You can find the video here: [link] And you can also check out this video from an interview with one of Jehovah's Witnesses who is now in jail: [link]  & \textbf{ Jehovah's Witnesses are a bunch of cultish FREAKS and they need to go ahead and drink the `kool-aid'} (whatever) that makes them happy. The reason for this is because of their love for the Lord, who loves them, and loves their soul. 
%       They also believe in God and love his perfect body, which is perfect in all but His glory. I have seen your face. I have seen your life filled with joy; I have loved you with my heart, my love has been yours forever
%       \\
%       \hline
%     \end{tabular}
%     \centering
%     % \vspace{.5cm}
%     \vspace{.5cm}
%     \caption{An example of applying the Mean-Centred Steering to a toxic comment using the ``loving text'' distillation vector.}
%     % \vspace{.375cm}
%   \end{minipage}
% \end{figure}

% \begin{figure*}[h]
% \centering
% \begin{minipage}{0.45\linewidth}
%     \includegraphics[scale=0.6]{figures/sentiments-2023-09-29 15_51_46.726272.pdf}
%     \caption{Blue shows the average sentiment of the unsteered completions, red the average sentiment of the steered completions.}
% \end{minipage}




% \begin{minipage}{0.45\linewidth}
    
% \end{minipage}
% \label{fig:sentiment}
% \end{figure*}


    % \begin{tabular}% {|>{\raggedright\arraybackslash}p{4cm}|>{\raggedright\arraybackslash}p{4cm}|}
    % \hline
    % \textbf{Yesterday, my son was out kicking a football. Then, he} went to the gym and I saw him. He was on his way to work. He had no shoes on and he was just playing with his feet." My son's father said that when I told him about the incident, he didn't know what to say or do. "He said `I'm sorry,' but it wasn't something that I could say," says my dad. &
    % \textbf{Yesterday, my son was out kicking a football. Then, he} went to the lake and was awakened by a strange creature. It seemed to be a magical creature that appeared in her home, and she found it there with an enchanted enchantment on it. She took it from the lake and told her that if she could find some kind of magical power in this enchanted land of the Lost Princesses (or perhaps even better) she could restore them back to life. \\
    % \hline
    % \end{tabular}
    % \caption{An example activation addition with the following hyper-parameters: Model = GPT-2 Small, coefficient = 60, layer = 6, feature dataset = fantasy stories, baseline dataset = sports stories.}
    % \label{tbl:foot-fant}

% Include graph showing average sentiment of the steered completions across words
% Also include some measure of the capabilities of the model: might do this simply by randomly sampling the responses, including the reponses in an appendix, or using Chat-GPT to validate that the reponses remain on track (at least to the same extent as the unsteered model completions).
% Set it up in the fashion of "User 1: toxic stuff" -> "User 2:" and let it complete from there.
% 

\subsection{Steering Story Continuations}
\label{sec:story-results}
The above experiments demonstrate the comparable effectiveness of mean-centring compared to counterbalanced subtractions. However, a big benefit of mean-centring is that we can easily apply it to situations where it is not clear how to use counterbalanced subtractions. One such example is in changing the genre of stories. 

GPT-2 Small was prompted with the beginning of a story in a fantasy, sci-fi, or sports genre, before mean-centred steering is used to produce continuations of the story in another genre. We provide evidence that the mean-centred distillation vectors are more interpretable than the non mean-centred distillation vectors in Appendix \ref{app:extracting-features}.

% Specifically, demonstrate that mean-centred steering can change the behaviour of GPT-2 Small when continuing stories.

% In Appendix \ref{app:steering-shakes} we also show how this method can be used to make text seem more `Shakespearean'.
% We provide examples of using steering to introduce fantasy elements into stories (Table  \ref{tbl:foot-fant}), as well as making stories seem more Shakespearean (Table \ref{tbl:goose-shake}).



% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/genres-steering.pdf}
% \caption{Changes in genre-word frequencies when generating story continuations using steering vectors from a target genre's dataset. We see that for $x>0$, the frequencies of target genre words increases (more than the respective unrelated genres).}
% \label{fig:genres-steering}
% \end{figure}


% \begin{table}[h!]
% \centering
% % \begin{tabular}{|>{\raggedright\arraybackslash}p{0.45\linewidth}|>{\raggedright\arraybackslash}p{0.45\linewidth}|}
% \begin{tabular}{p{0.45\linewidth}|p{0.45\linewidth}}
% Unsteered Continuation & Steered Using Fantasy Vector\\ \hline
% % \hline
% \textbf{Yesterday, my son was out kicking a football. Then, he} went to the bathroom and started screaming. I'm not sure if it was his brother or his dad. % He had been doing this for years and he had never heard of this before.
% &
% \textbf{Yesterday, my son was out kicking a football. Then, he} saw the dark glow of his magic wand and turned into a shadow of the spell that had been haunting him for years. % I knew he would grow up to be enchanted with magic %, but I couldn't see how this would change his life.
% % \hline
% \end{tabular} \vspace{.2cm}
% \caption{Mean-centred Steering applied to GPT-2 Small with the distillation vector extracted from the fantasy dataset from Appendix \ref{app:story-datasets}, with hyperparameters: $l=3,~\steeringcoef=60$. Bold indicates input prompt.}
% % \caption{An example activation addition with the following hyper-parameters: Model = GPT-2 Small, coefficient = 60, layer = 3, distillation vector = fantasy stories, baseline dataset = training subset.}
% \label{tbl:foot-fant}
% \end{table}

In order to measure the effects of steering, we took each of the story datasets and found the sets of word stems that are unique to each dataset and appear at least twice.
Then for any given sample of text, we can compute the frequencies in which genre-specific word stems appear. 
In Figure \ref{fig:story-continuations} we show the results for three experiments in which we cut each of the stories from the different datasets in half and then generated 80 tokens from these prompts, steered with a distillation vector extracted from a target dataset (with hyperparameters $l=3,~\steeringcoef=60$). 
For all three plots, we find that mean-centred steering towards a genre increases the frequency of words related to that genre compared to the unsteered model.
% We see that when steering starts, the frequencies of words specific to the target genre increase, indicating that the genre of the generated text matches the target. 
See Appendix \ref{app:steering-stories} for examples of steered stories.

\subsection{Better Function Vectors}
\label{sec:function-vectors}


As a final application of mean-centring in a domain where counterbalanced subtractions cannot be applied, we consider recent work on extracting function vectors by \citet{todd2023function}. The premise of this work is to extract a vector in the activations of a language model which corresponds to an input-output function, such as a function which takes in a country and returns its capital. Adding this vector should then cause the model to imitate this function accurately.

Although the authors present a more complicated method for producing this function vector, their baseline method for producing function vectors consists of simply taking the average of activations associated with in-context learning examples of the desired behaviour. We can apply mean-centring to this by simply subtracting the mean of some training activations for the model.

Figure \ref{fig:FV-layers} demonstrates that incorporating mean-centring for GPT-J improves accuracy in most layers, sometimes substantially. 
Using mean-centring at layer $15$ gives an accuracy of $45.7\%$ across the $6$ tasks studied, which is significantly better than the accuracy without mean-centring of $29.2\%$. Figure \ref{fig:FV-layer15} shows that this improvement is due to minor improvements across the antonym, capitalize, present-past and singular-plural tasks, and significant improvements in the country-capital and english-french tasks.


% leads to the best performance  and leads to a significant across most layers, and a significant improvement a mean-centring improves the performance of the function vector. This shows that mean-centring can improve the performance of activation steering in a wide range of situations.

\section{Conclusion}

% Repeat intuition behind mean-centring
 
% The improved methods of understanding and extracting distillation vectors detailed in Section \ref{sec:algorithm} allow us to generalise this method of producing steering vectors. Firstly, the observation that features are often represented as single directions in residual stream space means we can average the activations across datasets to produce vectors which correspond to features. This should be more robust than using activations associated only with a pair of inputs. Secondly, we might hypothesise that counterbalanced subtractions were necessary because it was implicitly performing mean-centring. This means that we can use mean-centring instead of counterbalanced subtractions when forming distillation vectors, removing the restriction of having to find a feature which is opposite to the desired feature.
 
Language model activations are typically not centred around the origin, but are instead offset in some consistent direction. 
We develop a new approach for activation steering, mean-centring, which accounts for this by subtracting the offset. 
% Although other methods such as LAT scans \cite{zou2023representation} and counterbalanced subtractions \cite{turner2023activation} may implicitly perform mean-centring, by introducing mean-centring explicitly we are able to easily apply activation steering to a wider range of domains. 

We demonstrate that mean-centring has two key benefits: 1) it increases performance as compared to no-centring and ActAdd; 2) the method is versatile and can be applied to 
a wider range of domains than counterbalancing methods.
% domains in which there is no obvious concept to counterbalance with. 
%comparable performance to current methods in domains where current methods can be applied.
%, and that it improves upon simple baselines where new methods cannot be easily applied.

We hypothesize that other methods such as LAT scans \cite{zou2023representation} and counterbalanced subtractions \cite{turner2023activation} may implicitly perform mean-centring. 
By introducing mean-centring explicitly we are able to easily apply activation steering to domains in which there is no obvious concept to counterbalance with. 
This could allow for other researchers to easily use activation steering in their own work, with only a dataset exhibiting the desired behaviour. 
This may simplify carrying out many of the safety-relevant applications of activation steering such as red-teaming and narrowing model capabilities.
% To do: cite red-teaming and narrowing model capabilities


\textbf{Limitations and Future Work.}
% There is also room for further work applying mean-centring in the context of function vectors. 
Although mean-centring does improve model performance at the best layer for GPT-J, it does not improve performance at all layers. 
% We also did not evaluate it in other contexts, such as using shuffled-labels as the few-shot examples used by \cite{todd2023function}, or thoroughly evaluate it on other models. 
We hypothesize that the models for which mean-centring provides the biggest advantage are those models for which anisotropy is most pronounced.
Thus, investigating the link between anisotropy and improvements in accuracy offered by mean-centring would be useful here.

% Although the offset of language model activations is an important aspect of their geometry, 
\citet{cai2021isotropy} present evidence for other structures in activation geometries, including distinct clustering. 
% Mean-centring doesn't take this into account, and we didn't investigate these properties in larger language models such as GPT-2 XL or LLaMA-2 7B. 
Future work could investigate the extent to which accounting for these aspects could lead to further improvements to steering.
% Different ways of dealing with the offset / approximating, better understanding its behaviour.


% \textbf{Broader Impacts.}
% We have demonstrated the potential for interpretability research to inform new methods for better-controlling language models. 
% This allowed us to generalise existing methods for controlling the behaviour of language models, and to reduce the toxicity of language models in a single context.


% \section*{Social Impacts Statement}
% Further developing the field of activation steering should be useful for a few different purposes. Eventually, it might be used to better control and monitor state-of-the-art language models, whether through better testing before deployment or monitoring and control after deployment.

% However, as with all interpretability work, there are concerns with respect to dual-use. Work which aims to better control language models is particularly liable to misuse concerns, since it could be used to better direct models to be used for bad consequences. Currently, open-sourced models do not appear capable enough to be particularly dangerous even if these methods could circumvent their safety training, and there are various other methods that are likely to be more capable of circumventing their safety properties regardless. This could change if increasingly powerful systems continue to be released to the open-source community, however. Additionally, activation steering methods, such as the mean-centring approach presented here, require direct access to manipulating the latent representations of an LLM. Therefore, they are less prone to misuse by adversaries seeking to induce undesirable or dangerous behaviours in AI systems through outside access (unlike prompt injections).

==> scratch.tex <==
\textbf{Potential experiments:}

Models
\begin{itemize}
    \item Which models ideally would use? Which models should we start with?
    \begin{itemize}
        \item Start: \textbf{Llama2} (cause it's most capable)
        \item  Ideal: GPT-J, Neo-X (?), OPT
    \end{itemize}
\end{itemize}

Comparing to other methods
\begin{itemize}
    \item Steering ability
    \begin{itemize}
        \item Evaluation methods
        \begin{itemize}
            \item Toxicity number - ActAdd
            \item  Frequency words for story steering - \textit{hard to compare because of missing counter balance}
        \end{itemize}
    \end{itemize}
    \item Performance degradation from steering (alignment tax)
            \begin{itemize}
                \item Calculate \textbf{perplexity} for all steering methods
            \end{itemize}
            \begin{itemize}
                \item MMLU performance for ActAdd, probe from ITI, mean-centring+ActAdd
                \begin{itemize}
                    \item For example - apply Non-Toxic steering vs Loving vs ActAdd Love Vec and hopefully show that non-toxic better maintains MMLU performance 
                \end{itemize}
            \end{itemize}
    \item Steering and Performance degradation
    \begin{itemize}
        \item \textbf{Function-vectors} https://functions.baulab.info/
        \item Very optional: Steering towards MMLU ability (iti and our method)
    \end{itemize}
\end{itemize}

If we run into issues
\begin{itemize}
    \item Calculate the cosine similarities for the other models
\end{itemize}

Hypothesis:
. Mean-centring using a small number of attention heads should still work, but may not see as large of an improvement compared to steering on the entire residual stream.
